Efficient Online Variational Estimation via Monte Carlo Sampling

This article addresses online variational estimation in parametric state-space models. We propose a new procedure for efficiently computing the evidence lower bound and its gradient in a streaming-data setting, where observations arrive sequentially. The algorithm allows for the simultaneous training of the model parameters and the distribution of the latent states given the observations. It is based on i.i.d. Monte Carlo sampling, coupled with a well-chosen deep architecture, enabling both computational efficiency and flexibility. The performance of the method is illustrated on both synthetic data and real-world air-quality data. The proposed approach is theoretically motivated by the existence of an asymptotic contrast function and the ergodicity of the underlying Markov chain, and applies more generally to the computation of additive expectations under posterior distributions in state-space models.

==> exp.tex <==
We now evaluate the proposed algorithm on several streaming data inference tasks.
Our goal is to demonstrate that the method can jointly learn both the latent posterior approximation and the model parameters in a fully sequential manner while requiring substantially less computation than existing online approaches (Table \ref{table:1_step_smoothing_chaotic_rnn}).

In all experiments, the variational filtering distributions $\vd{t}$ are chosen to be in the Gaussian family. For the non-linear models  (Sections~\ref{sec:xp:chaotic:rnn} and \ref{sec:exp_air_quality})
we implement the deterministic recursion $a_t = \amap{\parvar}(a_{t-1}, y_t)$ as an RNN, where both the update function $\amap{\parvar}$ and the parameter mapping $\fat$ are parameterized by MLPs with tanh activation functions.
The variational backward kernels are defined via the potentials $\fwdpot{t}$ in \eqref{eq:def:varbackwd}, which are parameterized by similar neural networks (except for the linear Gaussian case, where we exploit analytical conjugation to derive exact backward kernels).
In addition to this architecture, some control-variate tricks are implemented to reduce the variance of the gradient estimator (see details in Appendix~\ref{appdx:experiments} and ~\ref{appdx:full:algo}). 
% Finally, for all experiments, we use the Adam optimizer \cite{kingma2015adam} for training.


% We evaluate the proposed algorithm in the context of online variational learning for streaming data.
% Our goal is to demonstrate that the method can jointly learn both the latent posterior approximation and the model parameters in a fully sequential manner, requiring substantially less computation than existing online approaches (Table \ref{table:1_step_smoothing_chaotic_rnn}).
% To avoid the $O(N^2)$ complexity of computing full backward weights, we employ the backward sampling scheme of \citet{olsson2017efficient}.
% For the variational family, we utilize the general neural potential parameterization described in Section~\ref{sec:online_learning} for non-linear benchmarks.
% In contrast, for the Linear Gaussian experiment, we exploit exponential family conjugation to derive exact closed-form backward kernels. Additional implementation details and further experiments are reported in Appendix~\ref{sec:computational_considerations} and ~\ref{appdx:experiments}.



\subsection{Linear-Gaussian HMM}
\label{sec:LGHMM}
We first assess our algorithm on a linear Gaussian SSM. Consider $(X_t, Y_t)_{t \in \nset}$ in $\mathbb{R}^{\statedim}\times \mathbb{R}^{\obsdim}$, with $X_0 \sim \mathcal{N}(\mu_0, Q_0)$, $Y_0 = G X_0 + \varepsilon_0$, and, for all $t \in \nsetpos$,
\begin{align*}
    X_t &= F X_{t-1} + \nu_t, & \nu_t \overset{\text{i.i.d}}{\sim} \mathcal{N}(0, I_{\statedim}),\\
    Y_t &= G X_t + \varepsilon_t,& \varepsilon_t \overset{\text{i.i.d}}{\sim} \mathcal{N}(0,  I_{\obsdim}),
\end{align*}
where $\theta = (F, G)$ is the parameter to be learned.
% and $(\nu_t)_{t \in \nsetpos}$ and $(\varepsilon_t)_{t \in \nset}$ are i.i.d. standard Gaussian variables. 
In this case, the true smoothing distributions are Gaussian and can be computed via closed-form recursions (the Kalman smoother), providing an analytical reference for evaluation.
The variational family $\vd{0:t}$ is parameterized using Gaussian conditionals and marginals; see \Cref{sec:details:lin:Gauss} for details. 
%, then containing the true smoothing distribution.

% \paragraph{Online learning from streaming data. }
The first experiment is run with $\statedim=\obsdim=10$, and a sequence of $T=50000$ observations. 
Figure \ref{fig:training_lgm_50k} shows the evolution of the ELBO through the learning of ($\thp,\parvar$) as well as the posterior mean of the hidden states on a test sequence of observations never seen by the model. 
The right panel shows a particular dimension of the hidden state for the test sequence, as well as the learned posterior distribution at different iterations.  As the number of observations grows, our estimator learns a mapping that produces the true posterior distribution, corresponding to the oracle Kalman smoother. 
Figure~\ref{fig:lgm_mae_compare} shows the MAE in parameter estimation of $F$ (a) and $G$ (b). 
% A separate comparison of the learned model parameters (transition and emission maps) is shown in Figure~\ref{fig:lgm_mae_compare}. We benchmark against \citet{campbell2021online}. Both methods converge toward the true parameters, but 
Our method achieves lower error than the regression based method of \citet{campbell2021online} in roughly one quarter of the runtime when using $N=1000$ samples for the importance weights. 
Overall, these results highlight the computational efficiency of the proposed updates without compromising statistical accuracy.


\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{icml_linear_combined.pdf}
    \caption{(a) Evolution of $\approxELBO{t}/t$ during the online learning in the linear Gaussian SSM. Vertical lines indicate times at which state estimation is made on a test sequence. (b) State estimation on a test sequence (only one particular dimension is displayed).}
    \label{fig:training_lgm_50k}
\end{figure}


\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{icml_comparison_plot.pdf}
\caption{Model-parameter learning in the linear–Gaussian HMM.
Mean-absolute errors of the transition ($F$) and emission ($G$) matrices for our method and \citet{campbell2021online}.}
\label{fig:lgm_mae_compare}
\end{figure}



\subsection{Chaotic recurrent neural network.}
\label{sec:xp:chaotic:rnn}
We now consider the model used in \citet{campbell2021online}, where $X_0 \sim \mathcal{N}(0, Q)$, $Y_0 = X_0 + \varepsilon_0$, and, for $t \in \nsetpos$,
\begin{align*}
X_t &= X_{t-1} + \frac{\Delta}{\rho}\left(\gamma W \tanh{(X_{t-1})} - X_{t-1}\right) + \eta_t\eqsp,\\
Y_t &= X_t + \varepsilon_t \eqsp,
\end{align*}
where $(\eta_t)_{t \in \nsetpos}$ and $(\varepsilon_t)_{t \in \nset}$ are mutually independent sequences of i.i.d. $\mathcal{N}(0, Q)$ and   Student-$t$  random variables, respectively.   
We set $\statedim=\obsdim=5$, and the use same true parameters as \citet{campbell2021online} (see Appendix~\ref{appdx:chaotic:rnn}) and $N=500$ importance samples.

% \paragraph{Comparison with \citet{campbell2021online}.}
% The method proposed here differs from \citet{campbell2021online} mainly in how we approximate the backward statistic $\Hstat{t}$: we use a recursive sampling scheme rather than a regression-based estimator. To enable a fair comparison, we keep the generative parameters fixed exactly as in \citet{campbell2021online} and reproduce the 1-step smoothing evaluation of \citep[Appendix~B.2]{campbell2021online}.

% Specifically, we evaluate the ability of our approach to estimate the conditional laws of $X_{t-1}$ given $Y_{0:t}$ and of $X_t$ given $Y_{0:t}$ by computing $\expect{\vd{t-1:t}}{X_{t-1}}$ and $\expect{\vd{t}}{X_t}$, where $\parvar$ is trained using our amortized setting as described in  Section~\ref{sec:computational_considerations} and Appendix~\ref{appdx:details:non:amortized}). Implementation details are provided in Appendix~\ref{appdx:chaotic:rnn}.

% Table~\ref{table:1_step_smoothing_chaotic_rnn} reports the average 1-step smoothing and filtering errors,
% \begin{align*}
% \kappa^{(1)}_{T} &= \frac{1}{T-1}\sum_{t=1}^{T-1} \Big(\tfrac{1}{\statedim}\sum_{k=1}^{\statedim} (\mathbb{E}_{\vd{t-1:t}}[X_{t-1}^{(k)}] - x_{t-1}^{*(k)})^2\Big)^{\!1/2} \eqsp,\\
% \kappa^{(2)}_{T}&=\frac{1}{T}\sum_{t=1}^{T} \Big(\tfrac{1}{\statedim}\sum_{k=1}^{\statedim} (\mathbb{E}_{\vd{t}}[X_{t}^{(k)}] - x_{t}^{*(k)})^2\Big)^{\!1/2}\eqsp,
% \end{align*}
% for $\statedim=\obsdim=5$. We also report average computation time per gradient step over 8 runs with 8 different generative models (i.e., sequences). With comparable errors, our importance-sampling estimator of backward expectations is about $5\times$ faster than the regression approach.

\paragraph{Filtering and one-step smoothing}
To compare our method with the one of \citet{campbell2021online} on this model, we reproduce the 1-step smoothing experiment of their work \citep[Appendix~B.2]{campbell2021online}.
Specifically, we evaluate the ability of both approaches to estimate the conditional laws of $X_{t-1}$ given $Y_{0:t}$ and of $X_t$ given $Y_{0:t}$ by learning $\expect{\vd{t-1:t}}{X_{t-1}}$ and $\expect{\vd{t}}{X_t}$.
In order to perform the same comparison, we mimic the non-amortized framework of the original paper (details are provided Appendix~\ref{appdx:chaotic:rnn}).
Table~\ref{table:1_step_smoothing_chaotic_rnn} reports the 1-step smoothing and filtering errors as defined in Eqn.~\eqref{eq:1-step_error}.
We also report average computation time per gradient steps. 
With comparable errors,  
{\RMCVI}
% importance-sampling estimator of backward expectations 
is about $5$ times faster than the regression approach.

\begin{table}[b]
    \centering
    \small
    \begin{tabular}{||c||c|c|c||} 
        \hline
        Method & 1-Smooth. & Filt. & Time\\ [0.5ex] 
        \hline
        {\RMCVI} (ours) & 8.9 (0.2) & 10.3 (0.2) & 1 ms \\ 
        \hline
        \citet{campbell2021online} & 9.2 (0.2) & 10.3 (0.2) & 4.8 ms \\
        \hline
    \end{tabular}
    \caption{
    Time per gradient step, 1-step smoothing and filtering RMSE ($\times 10^{-2}$) (defined in Eqn.~\eqref{eq:1-step_error}) for the chaotic RNN.  
    % RMSE ($\times 10^{-2}$) of $\approxexpect{\vd{t-1:t}}{X_{t-1}}$  (Smooth.) and $\approxexpect{\vd{t}}{X_t}$ (Filt.) w.r.t.\ $x_{t-1}^*$ and $x_t^*$, with standard errors in parentheses, and average time per gradient step(see Eq.~\eqref{eq:1-step_error}).
    }
    \label{table:1_step_smoothing_chaotic_rnn}
\end{table}

\paragraph{Online learning.}
Moving beyond the fixed-parameter setting, we evaluate our method in a true streaming regime where both the variational parameters and selected generative parameters are learned online. 
Concretely, $T=5\times 10^5$ observations are processed with updates of the parameters 
% the nonlinear gain 
$\gamma$ and 
% the contraction/time–scale parameter 
$\rho$.
Figure~\ref{fig:chaotic_learning} (a) shows the MAE between parameter estimates and the true value. 
The  central panel shows the dynamics of $\approxELBO{t}/t$ with checkpoint markers, at which state estimation on held-out sequences is performed (right panel) for a specific state dimension. 
These results show that the proposed scheme remains stable and accurate while simultaneously learning $(\rho,\gamma)$ in this highly nonlinear regime.


\begin{figure*}[ht]
    \centering
    \includegraphics[width=\textwidth]{icml_chaotic_1x3.pdf}
    \caption{(a) Parameter MAE. (b) Approximate $\widetilde{\mathcal{L}}_t/t$ with checkpoint markers. (c) State estimation on a test sequence for one latent dimension. Colored lines/markers correspond to the same checkpoints.}
    \label{fig:chaotic_learning}
\end{figure*}



\subsection{Air-quality Data}
\label{sec:exp_air_quality}
We evaluate the framework on the UCI Air-Quality dataset \citep{uci_air_quality}, which consists of hourly averaged responses from a chemical sensor array alongside meteorological data. 
We process the data into an 8-dimensional observation vector $y_t \in \mathbb{R}^8$ spanning approximately one year ($T \approx 9,300$ steps). 
This benchmark is characterized by frequent periods of sensor failure, where valid signals are absent for extended durations. 
Rather than imputing these irregularities offline, we process the stream directly to rigorously test the method's ability to maintain coherent belief states during blackout periods. 
Visualizations of the data and more details on the signal characteristics and preprocessing are provided in Appendix~\ref{appdx:air_quality}.

% \PG{The data should be plot in Appendix \ref{appdx:air_quality}, it would avoid any long discourse. Do a plot with 8 panels sharing the same $x$-axis (the time) and showing the 8 signals. As such, we will easily see the censorship of the data} 

We model the air quality dynamics using a non-linear Gaussian SSM with residual transitions. 
Let $X_t \in \mathbb{R}^{5}$ and $Y_t \in \mathbb{R}^{8}$ denote the latent state and observations respectively. The generative process is defined as:
\begin{align*}
    X_t &= X_{t-1} + f_\theta(X_{t-1}) + \nu_t \eqsp, & \nu_t \sim \mathcal{N}(0, Q_\theta) \\
    Y_t &= g_\theta(X_t) + \varepsilon_t \eqsp, & \varepsilon_t \sim \mathcal{N}(0, R_\theta)
\end{align*}
where $f_\theta$ and $g_\theta$ are neural networks parameterized by $\theta$ (with tanh activations), and the noise terms have diagonal covariance matrices, which are also learned. Here we used $N=20$ importance samples for the Monte Carlo estimates. 
% Further details are provided in Appendix~\ref{appdx:air_quality}.


\paragraph{Online predictive performance.}
Our primary focus is the model's performance in an  online setting where all parameters must be learned from a cold start. 
We evaluate the model's ability to learn complex dynamics by measuring the one-step-ahead prediction RMSE on the five primary pollutants (CO, NO$_x$, NO$_2$, C$_6$H$_6$, O$_3$).
We compare our {\RMCVI} method against two baselines: a probabilistic online LSTM \citep{salinas2020deepar} with a Gaussian output  trained sequentially via maximum likelihood, and Online Variational SMC (OVSMC, \citealp{mastrototaro:olsson:2024}).

%Figure~\ref{fig:online_results} demonstrates the dual success of our approach. 
%As shown in Panel (a), our method effectively maximizes the ELBO over time, indicating stable convergence of the variational posterior. Simultaneously, Panel (b) reveals that our OVI model yields predictive performance comparable to the LSTM baseline and slightly better than the OVSMC method. This highlights that our method matches the forecasting capability of a standard autoregressive network, but does so by optimizing a variational lower bound. 
%Furthermore, OVI is computationally much faster than the particle-based OVSMC. Through our use of backward kernels, OVI provides a consistent smoothing posterior, offering a structural advantage over the purely filtering approach of OVSMC and the deterministic hidden states of the LSTM. Thus, we achieve the advantages of a learned latent structure in lower dimensions without losing predictive accuracy.

%\begin{figure}[ht]
%    \centering
%    \includegraphics[width=0.8\linewidth]{figures/figures_icml/icml_air_quality_final.pdf}
%    \vspace{-2mm}
%    \caption{\textbf{Simultaneous Variational Learning and Prediction.} 
%    (a) Smoothing reconstruction during sensor failure (black dotted). OVI (orange) recovers the Truth (gray) while LSTM (blue) overfits the corruption.
%    (b) Cumulative RMSE for one-step-ahead prediction averaged across all pollution features.}
%    \label{fig:online_results}
%\end{figure}


Figure~\ref{fig:online_results} demonstrates the robustness and accuracy of our approach. As shown in Panel (a), we introduce a smoothing experiment with artificial sensor failure. While the purely autoregressive LSTM is limited to filtering and thus tracks the corrupted signal, {\RMCVI} effectively recovers the underlying ground truth. Similarly, panel (b) confirms that {\RMCVI} matches the predictive performance of the LSTM and outperforms OVSMC. 
Thus, {\RMCVI} combines the forecasting power of autoregressive networks with the advantage of variational smoothing, all while maintaining lower computational costs than particle-based methods.



\begin{figure}[ht]
    \centering
    \includegraphics[width=0.8\linewidth]{icml_smoothingRMCV.pdf}
    \vspace{-2mm}
    \caption{\textbf{Simultaneous Variational Learning and Prediction.} 
    (a) Smoothing reconstruction during sensor failure (black dotted). {\RMCVI} (orange) recovers the Truth (gray) while LSTM (blue) overfits the corruption.
    (b) Cumulative RMSE for one-step-ahead prediction averaged across all pollution features.}
    \label{fig:online_results}
\end{figure}

==> intro.tex <==
This work considers \emph{state-space models} (SSMs) where the law of observations $(Y_t)_{t \in \nset}$ is governed by an unobserved, or `hidden', Markov chain $(X_t)_{t \in \nset}$, and the finite dimensional distributions of $(X_t, Y_t)_{t \in \nset}$ are given by parametric distributions indexed by $\thp \in \Theta$. Learning the parameter $\theta$ in this context is a complex task, as it usually requires access to the \textit{joint-smoothing distributions}, defined at time $t$ as the conditional distribution of the latent states $X_{0:t}$\footnote{$a_{u:v}$ is a short-hand notation for $(a_u,\ldots,a_v)$.} given the corresponding observations $Y_{0:t}$. 
This paper addresses the challenging problem of \emph{online estimation} in SSMs, which consists of sequentially learning both $\thp$ and the smoothing distributions as data stream in real time. 

A first possible approach to this task is based on sequential Monte Carlo (SMC) smoothing (see \citealp{chopin2020introduction} and the references therein). 
Such SMC-based methods for online learning come with strong theoretical guaranties \cite{le2013convergence,olsson2017efficient,tadic2020asymptotic,gao2025parameter}, but typically suffer from the curse of dimensionality in the state dimension. This recently motivated the use of variational inference (VI) \citep{blei2017} as an alternative, as VI has demonstrated strong empirical performance for online inference in large-scale settings, particularly through stochastic variational frameworks  \cite{hoffman2013stochastic, broderick2013streaming}. 

 Taking a variational approach, the smoothing distributions are approximated by simpler distributions, the \emph{variational distributions}, depending on some unknown parameter $\parvar\in\vparsp$. 
% This parameter is learned by maximizing the evidence lower bound (ELBO): 
% \begin{equation}
% \label{eq:ELBO}
% \ELBO{t} = \pE_{\vd{0:t}}\left[\log \frac{\jointd{0:t}(X_{0:t},Y_{0:t})}{ \vd{0:t}(X_{0:t})}\right] \eqsp,
% \end{equation}
% where $\jointd{0:t}$, defined in \eqref{eq:joint:ssm:dist}, is the joint distribution of the hidden states and the observations and $\thp$ is an unknown model parameter belonging to some parameter space $\thpsp$.
Both $\thp$ and $\parvar$ are then learned by maximizing a proxy of the log likelihood, the \emph{evidence lower bound} (ELBO), which is generally done using gradient ascent, thus requiring the computation of the ELBO's gradient. 
A key feature of these approaches is the choice of the variational distribution, which must be suited for online learning.
% The interest in online variational learning is strongly motivated by 
% First online variational procedures for SSMs rely on restrictive variational families, leading to biased approximations of the posterior distributions \cite{marino2018general,zhao2020variational}. 
\citet{campbell2021online} rely on structured variational distributions that both mimic the Markovian form of the  smoothing distributions (see \Cref{sec:model:background}) and are well suited to online learning. 
The authors explore online variational additive smoothing for the recursive computation of the ELBO and its gradients, using a Bellman-type recursion inspired by reinforcement learning and recursive maximum likelihood methods.  
% The authors rely on functional approximations of the conditional expectations at each timestep. 
A major limitation of this algorithm is that, \emph{at each iteration $t$}, it requires solving an inner optimization problem to learn a regression function serving as a proxy for a conditional expectation. This step can be computationally expensive and depends critically on the appropriate choice of the regression class.  
More broadly, a key drawback of existing online variational learning methods is the lack of theoretical guaranties for the proposed algorithms. 
% Most of the related works can be divided into two categories. 
% On the one hand, a majority of the methods are only amenable to offline estimation \citep{krishnan2017structured, lin2018variational, johnson2016}, \emph{i.e.}, they require prior access to the entire observation sequence $Y_{0:t}$ to compute the ELBO and its gradients. 
% On the other hand, some methods provide online procedures via alternative variational objectives that depart from \eqref{eq:ELBO} by making additional assumptions on the state dependencies under the variational law \citep{broderick2013streaming,Marino2018AGM,dowling2023real}. 

% In sequential variational inference, early works focus on offline scenarios with a forward variational factorization  \citep{johnson2016, krishnan2017structured, Lin2018VariationalMP, Marino2018AGM}. 
% One disadvantage of forward factorization is its incompatibility with the online setting. 
% On a distinct line of research \citep{Marino2018AGM, zhao2020variational, dowling2023real} opts to trade smoothing for filtering by targeting the marginal distributions at each timestep with variational distributions that depend only on the observations up to $t$. 

% Recently, \citet{chagneux2022amortized} established the first theoretical result on error control in sequential variational inference, building upon the backward variational factorization proposed by \citet{campbell2021online}. 


% Although the algorithm proposed by \citet{campbell2021online} outperforms several online filtering methods in SSM, its  recursions are very computationally intensive for large scale problems and  introduce an additional bias in the Monte Carlo estimator of the gradient. 
In this paper, we develop a theoretically grounded framework for online variational learning. 
Our approach is rooted in a stochastic approximation perspective, and, following \citet{mastrototaro:muller:olsson:2025}, we show that for a structured variational distributions parameterized by flexible function classes (such as deep neural networks), online variational learning amounts to maximizing a lower bound (COLBO) on the limiting time-normalized asymptotic log likelihood, also known as the asymptotic contrast function. Building on this theoretical framework, we first formulate an ideal---but generally intractable---stochastic approximation  algorithm that maximizes the COLBO, and then propose a Monte Carlo version of then same, using an efficient importance sampling approach that avoids any regression task and outperforms the algorithm of \citet{campbell2021online} in terms of computation time.
The main contributions of this paper can be summarized as follows:
% . We propose a Monte Carlo approximation of the theoretical updates using an efficient importance sampling approach that bypasses the regression task that is
% solved at each time step of previous methods.

\begin{itemize}
    \item We provide a theoretically grounded framework for online variational learning, showing that it can be viewed as Robbins---Monro algorithm.
    \item We propose a computationally efficient online estimator of the COLBO its gradient in the context of SSMs. In contrast to computationally intensive SMC or Markov chain Monte Carlo (MCMC) methods, our algorithm, which we refer to as \emph{Recursive Monte Carlo Variational Inference} (\RMCVI) to emphasize its iterative structure, relies on simple i.i.d. samples from the marginal variational distributions. 
     \item The proposed algorithm is not limited to the online computation and optimization of the COLBO and can be directly adapted to compute more general expectations, training losses, or gradients under distributions that admit a Markovian structure. 
    \item Experimentally, we demonstrate the performance of our estimator  both on synthetic and real world data.
\end{itemize}


% We refer the reader to \citep[Section 11]{douc2014nonlinear} for a presentation of the general concepts underlying SMC algorithms and to \citep{olsson2017efficient,gloaguen2022pseudo,dau2022complexity} for more recent work on this class of algorithms and their use for online smoothing. 
% Finally, we emphasize once again that the algorithm we propose is not limited to the computation of the ELBO and its gradient, but can be used for the online computation of smoothed expectations over \emph{arbitrary state functionals} of additive form.

\section{Related work}
Our methodology draws on recent advances in smoothing  methods for SSMs by (i) proposing a Monte Carlo approach for approximating conditional expectations  and (ii) relying on a structured variational family.
% However, a key difference is that all Monte Carlo samples are produced by i.i.d. sampling, which avoids the selection/mutation steps of SMC that lead to complex dependencies between samples over time. 

\emph{SMC for online learning in SSMs.} The original approaches to online smoothing is based on SMC methods. 
We refer the reader to \citep[Section~11]{douc2014nonlinear} for a presentation of the general concepts underlying SMC algorithms, and to \citet{olsson2017efficient,gloaguen2022pseudo,dau2022complexity} for more recent developments and applications of these methods to online smoothing.  
Theoretical guaranties for online optimization of the log-likelihood using SMC can be found in \cite{le2013convergence,olsson2017efficient,tadic2020asymptotic,gao2025parameter}.

\emph{Offline VI for SSMs.} Early works on VI for SSMs primarily focus on offline estimation \citep{johnson2016, krishnan2017structured, lin2018variational}, \emph{i.e.}, they require prior access to the entire observation sequence $Y_{0:t}$ in order to compute the gradients of the ELBO. These approaches rely on a \textit{forward} factorization of the variational distribution, which is incompatible with online learning. 

\emph{Online VI for SSMs.} \citet{Marino2018AGM, zhao2020variational, dowling2023real} opts to trade smoothing for filtering by targeting the marginal distributions at each timestep with variational distributions that depend only on observations up to $t$. 
By designing a new variational family, \citet{campbell2021online} show that the ELBO and its gradient can be recursively expressed via conditional expectations, providing a natural framework for online learning.  
The authors approximate these conditional expectations at each time step using functional approximations. 

\emph{Online Variational SMC.} A recent approach to improving SMC for online learning is to adapt the particle proposal dynamics by optimizing a variational objective \citep{zhao2022streaming, mastrototaro:olsson:2024, mastrototaro:muller:olsson:2025}. In this framework, the variational method aims to approximate the locally optimal proposal while simultaneously learning the model parameters, rather than targeting the full joint smoothing distribution. 

\emph{Theoretical guaranties for VI.} In the offline setting, \citet{chagneux2022amortized} established the first theoretical results on error control in VI for SSM, building on the variational family of \citet{campbell2021online}. 
Moreover, \citet{mastrototaro:muller:olsson:2025} provided an online variational SMC framework
% SMC-based framework 
% for online VI in SSMs 
that provably maximizes a well-defined asymptotic contrast function via stochastic approximation, which serves as the conceptual inspiration for our work.
%Moreover, 
%\citet{mastrototaro:muller:olsson:2025} provided an SMC-based framework for online VI in SSMs which provably maximizes a well-defined asymptotic contrast function using stochastic approximation.

==> model.tex <==
Consider an SSM $(X_t, Y_t)_{t \in \nset}$, where $(X_t)_{t \in \nset}$ is a discrete-time Markov chain on $\Xsp \eqdef \statesp$. 
The distribution of $X_0$ has density $\chi$ with respect to the Lebesgue measure $\mu$ and for all $t \in \nset$, the conditional distribution of $X_{t+1}$ given $X_{0:t}$ depends only on $X_t$ and has transition density $\hd{t}(X_{t},\cdot)$. 
In SSMs, it is assumed that the states of the Markov chain are only partially observed through an observation process $(Y_t)_{t \in \nset}$ taking on values in $\Ysp \eqdef \obssp$. 
For every $t \in \nset$,  the observations $Y_{0:t}$ are assumed to be conditionally independent given $X_{0:t}$ and such that  the conditional distribution of each $Y_s$, $s \in \intset{0}{t}$, given $X_{0:t}$ depends only on the corresponding $X_t$ and has density $\md{t}(X_t,\cdot)$ with respect to the Lebesgue measure. 
The model is then defined, for all $ t \in \nset$, by the joint distributions 
\begin{multline}
\label{eq:joint:ssm:dist}
\jointd{0:t}(x_{0:t},y_{0:t}) \eqdef \chi(x_0) \md{0}(x_0, y_0) \\
\times \prod_{s=1}^{t} \hd{s}(x_{s-1}, x_s)\md{s}(x_s, y_s) 
\end{multline}
of the hidden states and the observations.

A classical learning task in SSMs is \textit{state inference}, which consists of estimating the joint-smoothing distribution, \emph{i.e.} the conditional distribution of $X_{0:t}$ given $Y_{0:t}$, given by
$$
\post{0:t}(x_{0:t}) \eqdef \frac{\jointd{0:t}(x_{0:t},y_{0:t})}{\jointd{0:t}(y_{0:t})} \eqsp,
$$
where $\jointd{0:t}(y_{0:t}) \eqdef \int \jointd{0:t}(x_{0:t},y_{0:t}) \, \rmd x_{0:t} $ is the observed-data likelihood. %\propto$ means equality up to a multiplicative constant independent of $x_{0:t}$. 
The marginal of this joint distribution with respect to the state $x_t$ at time $t$ is known as the \textit{filtering distribution} at time $t$, and its density with respect to the Lebesgue measure is denoted by $\post{t}$. It is straightforward to show that the density of the joint-smoothing distribution satisfies the so-called \textit{backward decomposition}
\begin{equation}
\label{eq:post:backward:factorization}
    \post{0:t}(x_{0:t}) = \post{t}(x_t)\prod_{s=1}^{t} \backwd{s-1|s}(x_s, x_{s-1}) \eqsp, 
\end{equation}
where each \emph{backward kernel}
\begin{equation}
    \label{eq:true_backwd}
    \backwd{s-1|s}(x_s, x_{s-1}) \propto 
    \hd{s}(x_{s - 1},x_{s})\post{s - 1}(x_{s-1})
    %\frac{\hd{s}(x_{s - 1},x_{s})\post{s - 1}(x_{s-1})}{\int \hd{s}(x_{s-1},x_{s})\post{s - 1}(x_{s-1}) \, \rmd x_{s-1}} %,
\end{equation}
is the conditional probability density function of $X_{s-1}$ given $(X_{s}, Y_{0:s-1})$. The backward decomposition stems from the fact that the hidden process is still Markov when evolving conditionally on the observations, with time-inhomogeneous transition densities \eqref{eq:true_backwd}.  
However, since the filtering distributions are intractable, the backward kernels generally lack closed-form expressions. 

In variational approaches, the smoothing distribution $\post{0:t}$ is approximated by selecting a candidate from a parametric family $\{ \vd{0:t}\}_{\parvar \in \vparsp}$, known as the \textit{ variational family}, where $\vparsp$ is a parameter space. 
This parameter is learned jointly with $\thp$ by maximizing the ELBO 
\begin{equation}
\label{eq:ELBO}
\ELBO{t} = \pE_{\vd{0:t}}\left[\log \frac{\jointd{0:t}(X_{0:t},Y_{0:t})}{ \vd{0:t}(X_{0:t})}\right] \eqsp, 
\end{equation}
where $\pE_{\vd{0:t}}$ denotes expectation under $\vd{0:t}$. 
% where $\jointd{0:t}$, defined in \eqref{eq:joint:ssm:dist}, is the joint distribution of the hidden states and the observations and $\thp$ is an unknown model parameter belonging to some parameter space $\thpsp$.

Needless to say, the form of the variational family is crucial in this approach. 
Motivated by the backward decomposition, some works impose structure on the variational family through a factorization of $\vd{0:t}$. 
A variational counterpart of \eqref{eq:post:backward:factorization}, introduced by \citet{campbell2021online}, is given by
\begin{equation}
\label{eq:varpost:backward:factorization}
 \vd{0:t}(x_{0:t})=  \vd{t}(x_t)\prod_{s=1}^{t}\vd{s-1\vert s}(x_{s},x_{s - 1})\eqsp,
\end{equation}
where $\vd{t}$ (resp. $\vd{s - 1\vert s}(x_{s},\cdot)$) are user-designed probability density functions, the variational kernels, whose parameters are learned from data. 



A decisive advantage of this factorization is that it respects the true dependencies in \eqref{eq:post:backward:factorization}.
Moreover,  \citet{chagneux2022amortized} established an upper bound on the error when expectations with respect to the smoothing distribution are approximated by expectations with respect to variational 
distributions that satisfy this backward factorization.

\paragraph{Defining the variational distributions.}\label{sec:var_dist}
The variational inference framework requires the definition of the variational distributions involved in \eqref{eq:varpost:backward:factorization}, \textit{i.e.} the set of distributions $(\vd{t}, \vd{t| t+1})_{t\in \nset}$. We here define a new variational family in a recursive manner, with shared parameters over time. 
This new design based on backward factorization is efficient in terms of online parameter learning (as the number of parameters does not grow with $t$) and creates a link between variational kernels that will ensure an efficient importance sampling procedure in Section \ref{sec:MC:approach}. 

Our online learning challenge requires that variational distributions (i) can be recursively defined using streaming data $(y_t)_{t \in \nset}$, (ii) are related to each other to mimic the relation given by \eqref{eq:true_backwd} between the backward kernel and the filtering distribution, (iii) are easy to sample from to perform Monte Carlo approximations.
For this purpose, each $\vd{t}$ is chosen as a parametric distribution belonging to the exponential family (in our experiments, the Gaussian family in $\Xsp$), defined by some parameter $\eta_t$ belonging to a parameter space $\mathcal{E}$.
% denoted by $\mathsf{P} = \{P_\eta\}_{\eta \in \mathcal{E}}$, where $\eta$ is the corresponding natural parameter and $\mathcal{E}$ is the parameter space for this family 
% Let $\eta_t^\parvar$  be the parameter of $\vd{t}$.
More precisely, we define intermediate quantities $(a_t)_{t \in \nset}$  belonging to some user-defined space $\Asp$, initialized at some arbitrary value $a_0 \in \Asp$ and governed by a deterministic recursion $a_t = \amap{\parvar}(a_{t-1}, y_t)$. Based on these quantities, we let, for each $t$, $\eta_t = \fat(a_t)$. Here the mappings $\amap{\parvar}$ and $\fat$ are used-defined.
This framework creates a link between variational filtering distributions, in the spirit of the filtering recursions in SSMs.
The variational backward kernels are then defined from on the basis of this flow of distributions by setting, for all $t \in \nsetpos$, 
\begin{equation}
\label{eq:def:varbackwd}
\vd{t-1|t}(x_t, x_{t-1})  \propto \vd{t-1}(x_{t-1})\fwdpot{t}(x_{t-1}, x_t)\eqsp,
\end{equation}
where $(\fwdpot{t})_{t\geq 0}$ are potential functions on $\Xsp^2$ of form $\fwdpot{t}(x_{t-1}, x_t) = \exp( \langle \tilde{\eta}_t^{\parvar}(x_t), T(x_{t-1}) \rangle)$, 
%$$
%\begin{array}{lccl}
%\fwdpot{t}:&\statesp \times \statesp &\rightarrow& \rset_+  \\
%     & (x_{t-1}, x_t) &\mapsto&   \exp{(\tilde{\eta}_{t}^{\parvar}(x_t) \cdot T(x_{t-1}))}\eqsp,
%\end{array}
%$$
with $\tilde{\eta}_{t}^\parvar(x_t) = \fxt(x_t)$ and $T(x_{t-1})$ being a natural parameter and a sufficient statistic, respectively, for the chosen exponential family.
Eqn.~\eqref{eq:def:varbackwd} ensures that $\vd{t-1|t}(x_t, \cdot)$ will be a probability density function with natural parameter $\eta_{t-1|t}^\parvar = \eta_{t-1}^\parvar + \tilde{\eta}_t^\parvar$. 
In this convenient setting, the backward kernels $\vd{t-1|t}$ can have arbitrarily complex dependencies on $x_t$, while their densities are derived analytically from the potentials.
This enables straightforward Monte Carlo sampling procedures and direct computations of normalizing constants (which are required in our proposed algorithm, \emph{e.g.}, in \eqref{eq:backwardweights:offline} below), while at the same time avoiding the reduction of our variational kernels to mere transformations or linearizations (\emph{e.g.}, linear Gaussian kernels). 
In is important to note that the parameters of functions $\amap{\parvar},\fat,\fxt$ are shared across time, leading to an amortized framework. 
In our experiments, these functions are neural networks, and $\parvar$ are their weights.

% In the spirit of recurrent neural networks (RNN) we define intermediate quantities $a_t \in \mathsf{A}$ (where $\mathsf{A}$ is a user-defined space), such that\footnote{$\mathsf{MLP}$ is used to denote a multi-layer perceptron.} $a_t = \mathsf{MLP}^\parvar(a_{t-1}, y_t)$, and $\eta_t^\parvar = \mathsf{MLP}^{\parvar}(a_t)$. 
% Initialization is performed using a parameter $a_{-1}$, which can be fixed or learned.
% Note that the parameters $\parvar$ are shared across time, leading to a computationally efficient \textit{amortized scheme}. 
% The variational backward kernels are then defined from this flow of distributions by setting, for all $t \geq 1$, 
% \begin{equation}
% \label{eq:def:varbackwd}
% \vd{t-1|t}(x_t, x_{t-1})  \propto \vd{t-1}(x_{t-1})\fwdpot{t}(x_{t-1}, x_t)\eqsp,
% \end{equation}
% where $(\fwdpot{t})_{t\geq 0}$ are potential functions
% $$
% \begin{array}{lccl}
% \fwdpot{t}:&\statesp \times \statesp &\rightarrow& \rset_+  \\
%      & (x_{t-1}, x_t) &\mapsto&   \exp{(\tilde{\eta}_{t}^{\parvar}(x_t) \cdot T(x_{t-1}))}\eqsp,
% \end{array}
% $$
% with\footnote{We keep the generic $\parvar$ to avoid additional notations, but the MLP here is different from the one for $\vd{t}$.} $\tilde{\eta}_{t}^\parvar(x_t) = \mathsf{MLP}^\parvar(x_t)$ and $T(x_{t-1})$ are a natural parameter and a sufficient statistic for the family $\mathsf{P}$.
% Then, \eqref{eq:def:varbackwd} ensures that $\vd{t-1|t}(x_t, \cdot)$ will be a p.d.f.  in $\mathsf{P}$ with natural parameter $\eta_{t-1|t}^\parvar = \eta_{t-1}^\parvar + \tilde{\eta}_t^\parvar$. 
% In this convenient setting, the backward kernels $\vd{t-1|t}$ can have arbitrarily complex dependencies on $x_t$, while their densities are derived analytically from the potentials.
% This enables easy sampling for Monte Carlo procedures, and direct computations of normalizing constants (which are required in our proposed algorithm, for example, in Equation \eqref{eq:backwardweights:offline}), while at the same time avoiding the reduction of our variational kernels to mere transformations or linearizations (\emph{e.g.}, linear Gaussian kernels). 


% The learning of the variational parameters $\parvar$ is usually done via gradient ascent algorithms, which  require the calculation of the gradient of the ELBO with respect to the variational parameter.
% The next sections describe a new algorithm for the recursive approximation of this gradient.



==> online_learning.tex <==
\paragraph{The asymptotic contrast function and the COLBO.}
% In the following, we present an algorithm that incrementally learns optimal variational and model parameters $(\thp, \parvar)$ as new observations become available through a data stream $(Y_t)_{t \in \nset}$. 
% In the theoretical development of this algorithm, we assume that the observations are generated by an SSM, which may lie outside the parametric family introduced in \Cref{sec:model:background}. 
% In such cases, estimating the model parameters $\thp$ by repeatedly computing the full likelihood becomes impractical over time. 
In the context of maximum likelihood estimation, the online learning of an unknown model parameter $\thp$ is known as recursive maximum likelihood (RML) \cite{legland1997recursive}.
RML focuses on maximizing the \emph{asymptotic contrast function} $\contr(\thp) \eqdef \lim_{t\to\infty} t^{-1} \log p_\thp(Y_{0:t})$ (a.s.), which serves as a foundational objective in this setting. 
If the data are generated by an SSM belonging to the parametric family of interest, characterized by a ‘true’ parameter $\thp^\ast$, then, under suitable identifiability conditions, the asymptotic contrast is maximised at $\thp^\ast$. 
Consequently, the maximum likelihood estimator (MLE) is strongly consistent in the sense that it converges almost surely to $\thp^\ast$ as $t$ tends to infinity.

Since the asymptotic contrast $\contr(\thp)$ is intractable, we use a similar approach to that of \citet{mastrototaro:muller:olsson:2025} and instead aim to maximise online, with respect to $(\thp, \parvar)$, the \emph{contrast lower bound} (COLBO) given by 
\begin{equation} \label{eq:def:COLBO}
\COLBO(\thp, \parvar) \eqdef \lim_{t\to\infty} \frac{1}{t}\ELBO{t}
\leq \contr(\thp) \quad \mbox{(a.s.)}.
\end{equation}
% where $\ELBO{t}$ is the ELBO defined in \eqref{eq:ELBO}.
% Noticing that $\ELBO{t} = \sum_{s=0}^t \ELBO{s}-\ELBO{s-1}$ (with the convention $\ELBO{-1} = 0$), online learning of the COLBO mimicks the RML by performing gradient ascent, using $\grad_{\thp,\parvar}(\ELBO{s}-\ELBO{s-1})$ to build a sequence of estimates $(\thp_s,\parvar_s)_{s\geq 0}$.


\paragraph{Stochastic approximation viewpoint. }

Following standard RML ideas, online variational learning seek to maximize $\COLBO(\thp, \parvar)$ by updating $(\thp, \parvar)$ in the direction of its gradient. 
Because $\COLBO(\thp, \parvar)$ is defined as a long-run time average, it is natural to pursue a stochastic approximation approach with the goal of solving 
\(
\nabla_{\thp, \parvar}\,\COLBO(\thp, \parvar)=0.
\)
Indeed, defining $\gdiffELBO{t}%(Y_{0:t}) 
\eqdef \grad_{\thp,\parvar}\ELBO{t}-\grad_{\thp,\parvar}\ELBO{t-1}$, we may write  
%and noticing that $\ELBO{t} = \sum_{s=0}^t \ELBO{s}-\ELBO{s-1}$ (with the convention $\ELBO{-1} = 0$), we have that:
\begin{equation} \label{eq:grad:elbo:finite}
\frac{1}{t}\grad_{\thp,\parvar}\,\ELBO{t} = \frac{1}{t}\sum_{s=1}^t\gdiffELBO{s}
%(Y_{0:t})\,.
+ \frac{1}{t} \grad_{\thp,\parvar} \ELBO{0}. 
\end{equation}
% \[
% \begin{aligned}
% \label{eq:grad_COLBO:ergodic:limit}
% \lim_{t \to \infty} 
% \frac{1}{t}  \grad_{\thp,\parvar}\,\ELBO{t} 
% &=\; \lim_{t \to \infty} 
% \frac{1}{t} \sum_{s = 0}^{t}
% \left\lbrace\grad_{\thp,\parvar}\ELBO{s}-\grad_{\thp,\parvar}\ELBO{s-1}\right\rbrace \\
% &=\; \lim_{t \to \infty} 
% \frac{1}{t} \sum_{s = 0}^{t} \gdiffELBO{s} \\
% &\overset{\mathrm{a.s.}}{=}\; \grad_{\thp,\parvar}\,\COLBO(\thp, \parvar)
% =
% \int 
% \gdiffELBO{}(z)\,
% \Pi^{\thp, \parvar}\left(\rmd z \right).
% \end{aligned}
% \]
Interpreted through the lens of ergodic theory, it is tempting to see the long term limit of the right-hand side of \eqref{eq:grad:elbo:finite} as an expectation, allowing $\grad_{\thp,\parvar}\COLBO(\thp, \parvar)$ to be expressed as a \emph{mean field} (\emph{i.e.}, the deterministic drift) that governs the long-run behavior of Robbins--Monro stochastic updates. 
In this idealized framework, it is natural to use the observed gradient increments to build a sequence $(\thp_t,\parvar_t)_{t\in \nset}$  leading to an ideal procedure summarized in  Algorithm~\ref{alg:ideal}.
However, since each term $\gdiffELBO{s}$ depends on the whole historical record $Y_{0:s}$ and $(Y_t)_{t \in \nset}$ is not a Markov process, the existence of the limit of \eqref{eq:grad:elbo:finite} as $t$ tends to infinity is non-trivial.
Actually, to the best of our knowledge, no theoretical results exist justifying the existence of the COLBO objective \eqref{eq:def:COLBO} and its gradient, both of which are necessary to place this learning procedure on firm theoretical ground. 
% the COLBO can be rewritten, is optimized recusir, a natural update to asymptotically maximizes \eqref{eq:def:COLBO} is to update $(\thp,\parvar)$ using $\hGELBO{\thp,\parvar}{t} - \hGELBO{\thp,\parvar}{t-1}$.
In the coming sections we provide theoretical results motivating 
% the existence of the COLBO objective \eqref{eq:def:COLBO} and its gradient 
this existence
for the variational family of \Cref{sec:model:background} (Eqn.~\eqref{eq:varpost:backward:factorization} and \eqref{eq:def:varbackwd}). 
In particular, we show that the COLBO objective and its gradient can be justified via the law of large numbers, applied to a suitably constructed Markov chain. On the basis of this justification, Algorithm 1 can be motivated as a stochastic approximation scheme with state-dependent Markov noise. 

\begin{algorithm}[b]
\caption{Ideal algorithm (exact recursions)}
\label{alg:ideal}
\begin{algorithmic}[1]
\STATE \textbf{For each} \(t \in \nset\), at the arrival of $y_t$, using Prop. \ref{prp:elbo:grad:recursion}:
\STATE \quad Compute \(\Hstat{t},\Gstat{t},\Fstat{t}\).
\STATE \quad Compute 
         $\gELBOt{\thp}{t}{\thp_t,\parvar_t}$ and $\gELBOt{\parvar}{t}{\thp_t,\parvar_t}$.
\STATE \quad \textbf{Update:} 
\begin{align*}
    \parvar_{t+1} 
           &\gets \parvar_t 
           + \gamma^{\parvar}_{t+1}\left(\gELBOt{\parvar}{t}{\thp_t,\parvar_t}
- \gELBOt{\parvar}{t-1}{\thp_t,\parvar_t}\right)\,,\\
    \thp_{t+1} 
           &\gets \thp_t 
           + \gamma^{\thp}_{t+1}\left(\gELBOt{\thp}{t}{\thp_t,\parvar_t}
- \gELBOt{\thp}{t-1}{\thp_t,\parvar_t}\right)\,,      
\end{align*}
        where $(\gamma^{\thp}_{t+1}, \gamma^{\parvar}_{t+1})$ are learning rates satisfying the usual Robbins Monro conditions.
\end{algorithmic}
\end{algorithm}

\paragraph{Recursive expression of the ELBO and its gradient. }
In the following, we assume that we are given a sequence $(y_t)_{t \in \nset}$ of observations, and leave the dependence on these implicit in the notation. 
Write $\addfelbo{0}(x_{-1}, x_0) \eqdef \log(\chi(x_0) \md{0}(x_0, y_0))$, $q^{\parvar}_{-1\vert 0}(x_0, x_{-1})=1$
%$\addfelbo{0}(x_{-1}, x_{0}) =\log\ell_0(x_{-1}, x_0, y_0) $ 
and for $t \in \nsetpos$,
\begin{equation}
\label{eq:elbo:pair:terms}
\addfelbo{t}(x_{t-1}, x_{t}) \eqdef 
\log \left( \frac{\hd{t}(x_{t-1}, x_t)\md{t}(x_t, y_t)}{q^{\parvar}_{t-1\vert t}(x_t, x_{t-1})} \right),
%\log \frac{\qg{t}(x_{t-1}, %x_t, y_t)}{q^{\parvar}%_{t-1\vert t}(x_t, x_{t-1})}\,,
\end{equation}
which allows to rewrite the ELBO \eqref{eq:ELBO} as 
 $$
 \ELBO{t} = \pE_{ \vd{0:t}}\left[\sum_{s = 0}^t \addfelbo{s}(x_{s-1}, x_{s}) - \log \vd{t}(x_t)\right]\,.
 $$
 The following proposition provides recursive formulas for computing both the ELBO and its gradient. 
 For brevity, we let $\mathbb{E}^{\parvar,x_t}_{t-1|t}$ denote expectation under $\vd{t-1|t}(x_t, \cdot)$.  
\begin{proposition}
\label{prp:elbo:grad:recursion}
For every $t \in \nset$ and $(\thp, \parvar) \in \thpsp \times \vparsp$, the ELBO and its gradient are given by 
\begin{align*}
\ELBO{t} &= \expect{\vd{t}}{\Hstat{t}(X_t)} - \expect{\vd{t}}{\log\vd{t}(X_t)} \eqsp, \\
\grad_\parvar \ELBO{t}&= \expect{\vd{t}}{\grad_\parvar \log \vd{t}(X_t) \, \Hstat{t}(X_t) + \Gstat{t}(X_t)}%\label{eq:elbo:grad:update}
\eqsp, \\
\grad_\thp \ELBO{t} &= \expect{\vd{t}}{\Fstat{t}(X_t)} \eqsp,
\end{align*}
where the real-valued function $\Hstat{t}$ on $\Xsp$ and its gradients $\Gstat{t} \eqdef \grad_{\parvar} \Hstat{t}$ and 
$\Fstat{t} \eqdef \grad_{\thp} \Hstat{t}$ satisfy the recursions
\begin{align*}
     % \Hstat{t}(x_t) &=  
     % \pE_{\vd{t-1|t}(x_{t},\cdot)}\left[\Hstat{t-1}(X_{t-1}) + \addfelbo{t}(X_{t-1}, x_t)\right]\eqsp, \label{eq:Hstat:recursion} \\
     \Hstat{t}(x_t) &= \mathbb{E}^{\parvar,x_t}_{t-1|t}{\left[\Hstat{t-1}(X_{t-1}) + \addfelbo{t}(X_{t-1}, x_t)\right]}\\%\label{eq:Hstat:recursion}\\
     % \Gstat{t}(x_t) &= \mathbb{E}_{\vd{t-1|t}(x_{t},\cdot)}\left[\Gstat{t-1}\left(X_{t-1}\right) \right. \label{eq:Gstat:recursion}\\
     % &\left. 
     %  \hspace{1cm}+ \grad_\parvar \log \vd{t-1|t}(x_t, X_{t-1}) \right.\nonumber\\
     %  &\left. \hspace{1.5cm}\times\{\Hstat{t-1}(x_{t-1}) + \addfelbo{t}(x_{t-1}, x_t)
     % \} 
     % \right], \nonumber \\
     \Gstat{t}(x_t) &= \mathbb{E}^{\parvar,x_t}_{t-1|t}{\left[\Gstat{t-1}\left(X_{t-1}\right) + \grad_\parvar \log \vd{t-1|t}(x_t, X_{t-1}) \right.}\nonumber\\
      &{\left. \hspace{2.3cm}\times\{\Hstat{t-1}(x_{t-1}) + \addfelbo{t}(x_{t-1}, x_t)
     \} 
     \right]} \\%\label{eq:Gstat:recursion} \\
     % \Fstat{t}(x_t) &= \mathbb{E}_{\vd{t-1|t}(x_{t},\cdot)} \left[\Fstat{t-1}(X_{t-1}) + \grad_{\thp} \addfelbo{t}(X_{t-1}, x_t)\right]\eqsp, %\label{eq:Fstat:recursion}
     \Fstat{t}(x_t) &= \mathbb{E}^{\parvar,x_t}_{t-1|t} {\left[\Fstat{t-1}(X_{t-1}) + \grad_{\thp} \addfelbo{t}(X_{t-1}, x_t)\right]}\eqsp, %\label{eq:Fstat:recursion}
\end{align*}
with $\Hstat{0}(x_0) = \addfelbo{0}(x_{-1}, x_{0}),\Gstat{0}(x_0) = 0,$ and $\Fstat{0}(x_0)=\grad_\thp\addfelbo{0}(x_{-1}, x_{0})$. 
\end{proposition}

\begin{proof}
See \Cref{appdx:proof:prp:elbo:recursion}. 
\end{proof}

Proposition~\ref{prp:elbo:grad:recursion} is of twofold interest. First, it provides a recursive scheme for the online computation of the ELBO, which will lead to a learning algorithm in Section~\ref{sec:MC:approach}. Second, it highlights the natural quantities to consider when studying the existence of the COLBO objective and its gradient.
%The interest of Proposition~\ref{prp:elbo:grad:recursion} is twofold. 
%On the one hand, it provides a recursive scheme for online computation of the ELBO (which will lead to a learning algorithm in Section~\ref{sec:MC:approach}). 
%On the other hand, it emphasizes the natural quantities to consider for studying the existence of the COLBO and its gradient.

\paragraph{Existence of the COLBO.} From now on, we assume that the observed data is generated by some SSM $(X_t, Y_t)_{t \in \nset}$, which does not necessarily belong to the parametric family considered in  \Cref{sec:model:background}. Under this assumption, it is easy to see that also the process $(Z_t)_{t \in \nset}$, where $Z_t \eqdef (X_t, Y_t, \Hstat{t}, \Gstat{t}, \Fstat{t}, a_t)$, with $\Hstat{t}$, $\Gstat{t}$, and $\Fstat{t}$ being the functions defined recursively in \Cref{prp:elbo:grad:recursion} and $a_t$ being the intermediate quantities used in the parameterization of $\vd{t}$, is a Markov chain. 
The state space and Markov kernel of $(Z_t)_{t \in \nset}$ are denoted by $(\Zsp, \Zfd)$ and $\emk$, respectively (see  \Cref{app:extended-chain}, Eqn.~\eqref{eq:def:T}, for details).
The Markov property follows from the assumed SSM dynamics of $(X_t, Y_t)_{t \in \nset}$, along with the fact that the updates of Proposition \ref{prp:elbo:grad:recursion} 
% in \eqref{eq:Hstat:recursion} and \eqref{eq:Gstat:recursion}
, as well as the update of $a_t$ from $a_{t - 1}$, are performed recursively based on the current observation $Y_t$. Denote also by $\S$ the Markov kernel of the marginal chain $(X_t, Y_t, a_t)_{t \in \nset}$. We will establish the exponential forgetting of the extended chain $(Z_t)_{t \in \nset}$ under the following assumptions.
\begin{assumption} \label{ass:unif:erg:xya:main}
    %For every $(\thp, \parvar) \in \Theta \times \vparsp$, the chain $(Z_t)_{t \in \nset}$ is uniformly ergodic with mixing rate $\rho^{\thp, \parvar} \in (0, 1)$. In addition, $\inf_{(\thp, \parvar) \in \Theta \times \vparsp} \rho^{\thp, \parvar} > 0$. 
    There exist $\pi \in \probmeas(\Xfd \tensprod \Yfd \tensprod \Afd)$ and $\alpha \in (0, 1)$ such that for every $t \in \nsetpos$, $\parvar \in \Phi$, and $(x, y, a) \in \Xsp \times \Ysp \times \Asp$,  
    $$
    \| (\S)^t(x, y, a) - \pi \|_{\mathsf{TV}} \leq \mixrt^t. 
    $$
\end{assumption}

\Cref{ass:unif:erg:xya:main} is discussed in \Cref{sec:discussion:unif:erg:xya}. The following assumptions are purely technical. 

\begin{assumption} \label{ass:grad:unif:bound:main}
    There exists $c \in \rsetpos$ such that for every $\parvar \in \Phi$, $a_t \in \Asp$, and $(x_{s + 1}, y_{s + 1}) \in \Xsp \times \Ysp$,     
    \begin{itemize}
        \item[(i)] $\mathbb{E}^{\parvar,x_{s+1}}_{s|s+1}\left[| \grad_\parvar \log \vd{s|s + 1}(x_{s + 1}, X_s) |^2 \right] \leq c^2$, 
        \item[(ii)] $\mathbb{E}^{\parvar,x_{s+1}}_{s|s+1}\left[|\addfelbo{s}(X_s, x_{s + 1})|^2 \,\right] \leq c^2$,  
        \item[(iii)] $\mathbb{E}^{\parvar,x_{s+1}}_{s|s+1}\left[ | \grad_\thp \addfelbo{s}(X_s, x_{s + 1}) | \right] \leq c$. 
    \end{itemize}
\end{assumption}

\begin{assumption}\label{ass:bounded-pot:main}
There exist constants $0<\varepsilon^{-}<\varepsilon^{+}<\infty$ such that, for every $t\in \nsetpos$, $(x_{t-1}, x_t) \in\X^2$, and $\parvar\in\Phi$,
\[
   \varepsilon^{-} \le \fwdpot{t}(x_{t-1},x_t) \le \varepsilon^{+}.
\]
\end{assumption}
%Let $\lip(\Zfd)$ be the set of $f \in \mf(\Zfd)$ for which 

The following theorem establishes the geometric ergodicity of the extended Markov chain, if not for all $f$ in the space $ \bmf(\Zfd)$ of bounded measurable functions on $\Zsp$, so at least for a subclass $\lip(\Zfd) \subset \bmf(\Zfd)$ of Lipschitz functions. More precisely, $f \in \lip(\Zfd)$ if there exists $\varphi \in \bmf(\Xfd \tensprod \Yfd \tensprod \Afd)$ such that for every $(x, y, a, h, h', u, u', v, v') \in \Xsp \times \Ysp \times \Asp \times \bmf(\Xfd)^6$, writing $\mathsf{s} = (x, y, a)$,
    \begin{itemize}
        %\item[(i)] $f(\cdot, h, u, v) \in \lip_1(\Xfd \tensprod \Yfd \tensprod \Afd)$, 
        \item[(i)] $|f(\mathsf{s}, h, u, v)| \leq \varphi(\mathsf{s})$, 
        \item[(ii)] $|f(\mathsf{s}, h, u, v) - f(\mathsf{s}, h', u', v')| \\ 
        \leq \varphi(\mathsf{s}) \left( \oscnorm(h - h') + \oscnorm(u - u') + \oscnorm(v - v') \right).$ 
    \end{itemize}

%described in detail in \Cref{app:extended-chain}. 
\begin{theorem}[Geometric ergodicity of $(Z_t)_{t \in \nset}$]
\label{th:main}
Assume  \ref{ass:unif:erg:xya:main}--\ref{ass:bounded-pot:main}. Then there exist $\rho \in (0, 1)$ and a functional $\statemap : \bmf(\Xfd)^6 \to \rsetpos$ such that for every $(\thp, \parvar) \in \Theta \times \vparsp$, $t \in \nset$, $f \in \lip(\Zfd)$, $z = (x_0, y_0, a_0, h_0, u_0, v_0) \in \Zsp$, and $z' = (x'_0, y'_0, a'_0, h'_0, u'_0, v'_0) \in \Zsp$,  
    \begin{multline}  \label{eq:K:diff:bound:final}
    |(\K)^t f(z) - (\K)^t f(z')| \\
    \leq  \statemap(h_0, h'_0, u_0, u'_0, v_0, v'_0) \| \varphi \|_\infty \rho^t.     
    \end{multline}
    Moreover, there exists a functional $\bar{\statemap} : \bmf(\Xfd)^3 \to \rsetpos$ and a kernel $\Pi^{\thp, \parvar}$ such that for every $f \in \lip(\Zfd)$, $\Pi^{\thp, \parvar} f$ is constant and for every $t \in \nset$ and $z = (x_0, y_0, a_0, h_0, u_0, v_0) \in \Zsp$, 
    \begin{equation} \label{eq:erg:extended:chain}
    |(\K)^t f(z) - \Pi^{\thp, \parvar} f| \leq \bar{\statemap}(h_0, u_0, v_0) \| \varphi \|_\infty \rho^t.   
    \end{equation}
    %where 
    %\begin{multline*} 
     %   \bar{\statemap}(h_0, u_0, v_0) \\
     %   \eqdef \frac{1}{1 - \rho} \int \statemap(h_0, h'_0, u_0, u'_0, v_0, v'_0) \, \K(z, \rmd z'). 
    %\end{multline*}
\end{theorem}
\begin{proof}
See \Cref{app:extended-chain}.
\end{proof}

Although the contraction \eqref{eq:erg:extended:chain} does not hold in the total variation norm (due to the restriction to test functions in $\lip(\Zfd)$), the quantity $\Pi^{\thp, \parvar}$ provided by the same theorem can be regarded as a candidate for the unique stationary distribution of $(Z_t)_{t \in \nset}$. Moreover, by \Cref{prp:elbo:grad:recursion}, each term $\gdiffELBO{s} = \gdiffELBO[Z_{s - 1:s}]{}$ depends explicitly on the consecutive states $Z_{s - 1:s}$ of the extended chain. By the law of large numbers for Markov chains, we may expect that (a.s.),  
\begin{equation} \label{eq:mean:field:representation}
    \lim_{t \to \infty} \frac{1}{t} \, \grad_{\thp,\parvar} \ELBO{t} %\overset{\text{a.s.}}{=}
    =
    \iint \gdiffELBO[z, z']{} \, 
    %\Pi^{\thp, \parvar} \tensprod \K(\rmd(z, z'))
    \Pi^{\thp, \parvar}(\rmd z) \, \K(z, \rmd z').   
\end{equation}
Letting the limit \eqref{eq:mean:field:representation} serve as the mean field of a stochastic approximation scheme with state-dependent Markov noise \citep[see][Case~2]{karimi:etal:2019}, a recursive Robbins--Monro algorithm finding a stationary point of the COLBO gradient is given by
$$
(\theta_{t + 1}, \parvar_{t + 1}) \gets (\theta_t, \parvar_t) + \gamma_{t + 1} \mathcal{G}^{\thp_t, \parvar_t} \langle Z_{t - 1}, Z_t \rangle,  
$$
and $Z_{t + 1} \sim T^{\thp_{t + 1}, \parvar_{t + 1}}(Z_t, \cdot)$, where  $(\gamma_t)_{t \in \nsetpos}$ is a sequence of step sizes satisfying the usual assumptions. This procedure is summarized in \Cref{alg:ideal}, which uses distinct step-size sequences $(\gamma_t^\thp)_{t \in \nsetpos}$ and $(\gamma_t^\parvar)_{t \in \nsetpos}$ for updating the model and variational parameters. 








% Each incremental update can be computed efficiently by using the recursive updates of the extended state variables (Sec.~\ref{sec:main:algorithm}). 

% \paragraph{Purely Theoretical Algorithm (Exact Recursions)}
% In an idealized scenario, one may compute all conditional expectations in the underlying recursions \emph{exactly} under $\vd{t-1\mid t}$. This yields closed-form expressions for 
% \(\Hstat{t},\Gstat{t},\Fstat{t}\). 
% Substituting these into the update rule above directly provides 
% \(\grad_{\thp, \parvar}\,\ELBO{t}\), 
% so the online parameter update becomes exact. 







% In  this algorithm, $\grad \log \vd[\parvar_t]{t}(\sample{t}{i})$ should be understood as $\grad_\parvar \log \vd[\parvar]{t}(\sample{t}{i}) |_{\parvar = \parvar_t}$ (and similar for other quantities). Equations \eqref{eq:approx:Hstat:online}--\eqref{eq:approx:Gstat:online} 
% are almost identical to \eqref{eq:approx:Hstat:offline}--\eqref{eq:approx:Gstat:offline}.
% The crucial difference is the presence of quantities on the right-hand sides of \eqref{eq:approx:Hstat:online}--\eqref{eq:approx:Gstat:online} that are calculated using $\parvar_{t - 1}$ and thus introduce new approximations.
% These approximations, which are usually made in recursive maximum likelihood settings, are essential for the practical implementation of online learning.
%Although these approximations make the theoretical analysis more complex, in practice they lead to good results, as we shall see in Section \ref{sec:experiments}.

==> online_monte_carlo_approximation.tex <==

We now derive a practical version of the ideal Algorithm~\ref{alg:ideal}.  \Cref{prp:elbo:grad:recursion} suggests that it is possible to estimate the ELBO and its gradient recursively. The key feature of our Monte Carlo algorithm is that each conditional expectation in the recursion only needs to be estimated on a \textit{finite support}, bypassing the regression step required at each time step in  \citet{campbell2021online}. This results in a more efficient procedure, as confirmed empirically in Section \ref{sec:xp:chaotic:rnn}. The algorithm proceeds as follows:

First, sample $\lbrace \sample{0}{i} \rbrace_{i = 1}^N\overset{\text{i.i.d.}}{\sim} \vd{0}$, and set 
% $\approxHstat{0}{i} = \Hstat{0}(\sample{0}{i})$, $\approxGstat{0}{i} = \Gstat{0}(\sample{0}{i}), \approxFstat{0}{i} = \Fstat{0}(\sample{0}{i}).$
$$
\approxHstat{0}{i} = \Hstat{0}(\sample{0}{i}), \quad \approxGstat{0}{i} = \Gstat{0}(\sample{0}{i}), \quad \approxFstat{0}{i} = \Fstat{0}(\sample{0}{i})\,.
$$ 
At time $t \in \nsetpos$, having access to a Monte Carlo sample $\lbrace \sample{t - 1}{i} \rbrace_{1 = i}^N$ from $\vd{t - 1}$ and approximations $\approxHstat{t - 1}{i},\approxGstat{t - 1}{i},\approxFstat{t - 1}{i}$ of $\Hstat{t - 1}(\sample{t - 1}{i}),\Gstat{t - 1}(\sample{t - 1}{i}), \Fstat{t - 1}(\sample{t - 1}{i})$, respectively, 
sample independently $\lbrace \sample{t}{i} \rbrace_{i = 1}^N$ from $\vd{t}$ and update 
\begin{align}
\approxHstat{t}{i} =& \sum_{j=1}^N \nrmbackwdweight{t}{i,j}
\left(\approxHstat{t-1}{j} + \addfelbo{t}(\sample{t-1}{j}, \sample{t}{i}) \right), \label{eq:approx:Hstat:offline}\\ 
\approxGstat{t}{i} =& \sum_{i=1}^N \nrmbackwdweight{t}{i,j}\left\{\approxGstat{t - 1}{j} + \grad_\parvar \log \vd{t-1|t}(\xi_{t}^i, \xi_{t-1}^j)\right.\nonumber\\
& \hspace{1.5cm}\left. \times \left( \approxHstat{t-1}{j} + \addfelbo{t}(\xi_{t-1}^j, \xi_t^i) \right)\right\},  \label{eq:approx:Gstat:offline}\\
\approxFstat{t}{i} =& \sum_{i=1}^N \nrmbackwdweight{t}{i,j}\left(\approxFstat{t - 1}{j} + \grad_\thp \addfelbo{t}(\sample{t-1}{j}, \sample{t}{i})\right),  \label{eq:approx:Fstat:offline}
\end{align}
where
\begin{equation}
    \label{eq:backwardweights:offline}
    \nrmbackwdweight{t}{i,j} \eqdef \frac{\vd{t-1 \vert t}(\sample{t}{i}, \sample{t-1}{j})/\vd{t-1}(\sample{t-1}{j})}{\sum_{k=1}^N \vd{t-1 \vert t}(\sample{t}{i}, \sample{t-1}{k})/\vd{t-1}(\sample{t-1}{k})}\eqsp.
\end{equation}

Estimators (\ref{eq:approx:Hstat:offline}--\ref{eq:approx:Fstat:offline}) are \textit{self-normalized importance sampling} estimators  of the updates of Proposition \ref{prp:elbo:grad:recursion}, and \eqref{eq:backwardweights:offline} provides the (shared) importance weights of these estimators. 
Note that we cannot perform direct Monte Carlo approximation on the basis of samples from $\vd{t-1\vert t}(\sample{t}{i},\cdot)$, as we would not have access to any approximations of the values of the functionals $\Hstat{t-1}$ and $\Gstat{t-1}$ at the sampled points. 
The use of importance sampling is therefore a  prerequisite for updating the approximations. 
Moreover, note that the design of variational distributions imposed by \eqref{eq:def:varbackwd} creates a link between the the target $\vd{t - 1\vert t}$ distribution and $\vd{t}$, making the latter a natural proposal distribution.

Once $\{(\approxHstat{t}{i},\approxGstat{t}{i},\approxFstat{t}{i})\}_{i = 1}^N$ are computed, approximations of the ELBO and its gradient at time $t$ are obtained by 
\begin{align}
\approxELBO{t} &= \frac{1}{N}\sum_{i = 1}^N\left( \approxHstat{t}{i} - \log\vd{t}(\sample{t}{i})\right),\label{eq:approx:ELBO}\\
\hGELBO{\parvar}{t} &= \frac{1}{N}\sum_{i = 1}^{N}\left( \grad_\parvar \log \vd{t}(\sample{t}{i})  \approxHstat{t}{i} + \approxGstat{t}{i}\right), \label{eq:approx:grad:phi}\\
\hGELBO{\thp}{t} &= \frac{1}{N}\sum_{i = 1}^{N}\approxFstat{t}{i}. \label{eq:approx:grad:theta}
\end{align}
The full procedure, which we refer to as {\RMCVI} (Recursive Monte Carlo Variational Inference), is detailed in \Cref{alg:onlinenabla} in \Cref{appdx:alg}. 
Appendix \ref{appdx:full:algo} provides refinements to increase computational efficiency and reduce the variance of the gradient estimator.
It is worth noting that {\RMCVI} computes estimated gradients using both $(\parvar_t,\thp_t)$ and $(\parvar_{t-1},\thp_{t-1})$ (Eqns.~(\ref{eq:approx:update:phi}--\ref{eq:approx:update:theta}), Appendix~\ref{appdx:alg}),  which introduces a deviation from the ideal updates of Algorithm~\ref{alg:ideal}.
Such approximations---commonly employed in RML settings---are crucial for enabling a feasible  practical online implementation.
% \begin{algorithm}[H]
% \caption{Online gradient estimator}\label{alg:onlinenabla}
% \begin{algorithmic}
% \STATE {\bfseries Input:} initial parameter estimate $\lambda_0$, step sizes $\{\gamma_t\}_{t \geqslant 1}$.
% \STATE Sample $\lbrace \sample{0}{i} \rbrace_{i = 1}^N$ independently from $\vd[\parvar_0]{0}$\; 
% \STATE set $\approxHstat[\parvar_0]{0}{i} \gets \Hstat[\parvar_0]{0}(\sample{0}{i})$ and $\approxGstat[\parvar_0]{0}{i} \gets 0$\;
% \STATE set 
% $\widehat{\grad} \ELBO[\parvar_0]{0} \gets N^{-1} \sum_{i = 1}^{N} \grad \log \vd[\parvar_0]{0}(\sample{0}{i}) \approxHstat[\parvar_0]{0}{i} + \approxGstat[\parvar_0]{0}{i}$\;
% \STATE update $\parvar_1 \gets \parvar_0 + \gamma_1\widehat{\grad} \ELBO[\parvar_0]{0}$\;
% \FOR{$t \leftarrow 1$ to $n-1$}
% \STATE sample $\lbrace \sample{t}{i} \rbrace_{i = 1}^N$ independently from $\vd[\parvar_t]{t}$\; 
% \STATE set 
% \begin{equation}
% \label{eq:backwardweights:online}
%     \nrmbackwdweight[\parvar_t]{t}{i,j} \gets \frac{\vd[\parvar_{t}]{t-1 \vert t}(\sample{t}{i}, \sample{t-1}{j})/\vd[\parvar_{t - 1}]{t-1}(\sample{t-1}{j})}{\sum_{k=1}^N \vd[\parvar_{t}]{t-1 \vert t}(\sample{t}{i}, \sample{t-1}{k})/\vd[\parvar_{t - 1}]{t-1}(\sample{t-1}{k})} \ ; 
% \end{equation}
% \STATE update 
% \begin{align}
% \approxHstat[\parvar_t]{t}{i} &\gets \sum_{j=1}^N \nrmbackwdweight[\parvar_t]{t}{i,j}
% \left(\approxHstat[\parvar_{t-1}]{t-1}{j} + \addfelbo[\parvar_t]{t}(\sample{t-1}{j}, \sample{t}{i}) \right) \eqsp, \label{eq:approx:Hstat:online}\\ 
% \approxGstat[\parvar_t]{t}{i} &\gets \sum_{i=1}^N \nrmbackwdweight[\parvar_t]{t}{i,j}\left\{\approxGstat[\parvar_{t-1}]{t - 1}{j} + \grad \log \vd[\parvar_{t}]{t-1|t}(\xi_{t}^i, \xi_{t-1}^j)  \left( \approxHstat[\parvar_{t - 1}]{t-1}{j} + \addfelbo[\parvar_t]{t}(\xi_{t-1}^j, \xi_t^i) \right)\right\}\eqsp;  \label{eq:approx:Gstat:online}
% \end{align}
% \STATE set 
% $
% \displaystyle \widehat{\grad} \ELBO[\parvar_t]{t} \gets \frac{1}{N} \sum_{i = 1}^{N} \left( \grad \log \vd[\parvar_t]{t}(\sample{t}{i})  \approxHstat[\parvar_t]{t}{i} + \approxGstat[\parvar_t]{t}{i} \right)
% $\;
% \STATE update $\parvar_{t+1} \gets  \parvar_t + \gamma_{t+1}\left(\widehat{\grad}_\parvar \ELBO[\parvar_t]{t} - \widehat{\grad}_\parvar \ELBO[\parvar_{t-1}]{t-1}\right)\eqsp;$
% \ENDFOR
% \end{algorithmic}
% \end{algorithm}


% \textbf{Note.} This is the algorithm with the extra Monte Carlo step, where the previous gradient is never used for the parameter update steps. It corresponds to the update described in Equation~\eqref{eq:robbins-monro:scheme}.




==> recursions.tex <==
\paragraph{Notations. } For all distribution $\mu$, we write $\mathbb{E}_\mu$ the expectation under $\mu$. For all $1\leqslant t\leqslant T$ and all $x\in\mathbb{R}^d$, we use the notation $\mathbb{E}^{\parvar,x_t}_{t-1|t}$ for $\mathbb{E}_{q^{\parvar}_{t-1|t}(x,\cdot)}$.

\paragraph{Recursive expression of the ELBO and its gradient}
In the following we assume that we are given a sequence $(y_t)_{t \geqslant 0}$ of observations, and leave the dependence on these implicit in the notation. 
Write $\addfelbo{0}(x_{-1}, x_0) \eqdef \log(\chi(x_0) \md{0}(x_0, y_0))$ 
%$\addfelbo{0}(x_{-1}, x_{0}) =\log\ell_0(x_{-1}, x_0, y_0) $ 
and for $t>0$,
\begin{equation}
\label{eq:elbo:pair:terms}
\addfelbo{t}(x_{t-1}, x_{t}) = 
\log \left( \frac{\hd{t}(x_{t-1}, x_t)\md{t}(x_t, y_t)}{q^{\parvar}_{t-1\vert t}(x_t, x_{t-1})} \right),
%\log \frac{\qg{t}(x_{t-1}, %x_t, y_t)}{q^{\parvar}%_{t-1\vert t}(x_t, x_{t-1})}\,,
\end{equation}
which allows to rewrite Equation \eqref{eq:ELBO} as 
 $$
 \ELBO{t} = \pE_{ \vd{0:t}}\left[\sum_{s = 0}^t \addfelbo{s}(x_{s-1}, x_{s}) - \log \vd{t}(X_t)\right]\,.
 $$
 The following Proposition gives the equations to compute recursively both the ELBO and its gradient.

\begin{proposition}
\label{prp:elbo:grad:recursion}
For every $t \geqslant 0$, $\thp\in\thpsp$ and $\parvar \in  \vparsp$, the ELBO \eqref{eq:ELBO} and its gradient are given by 
\begin{align*}
\ELBO{t} &= \expect{\vd{t}}{\Hstat{t}(X_t)} - \expect{\vd{t}}{\log\vd{t}(X_t)} \eqsp, \\
\grad_\parvar \ELBO{t}&= \expect{\vd{t}}{\grad_\parvar \log \vd{t}(X_t) \, \Hstat{t}(X_t) + \Gstat{t}(X_t)}%\label{eq:elbo:grad:update}
\eqsp, \\
\grad_\thp \ELBO{t} &= \expect{\vd{t}}{\Fstat{t}(X_t)} \eqsp,
\end{align*}
where the function $\Hstat{t} : \statesp \to \mathbb{R}$ and its gradients $\Gstat{t}~\eqdef~\grad_{\parvar}~\Hstat{t}$ and 
$\Fstat{t}~\eqdef~\grad_{\thp} \Hstat{t}$ satisfy the recursions
\begin{align*}
     % \Hstat{t}(x_t) &=  
     % \pE_{\vd{t-1|t}(x_{t},\cdot)}\left[\Hstat{t-1}(X_{t-1}) + \addfelbo{t}(X_{t-1}, x_t)\right]\eqsp, \label{eq:Hstat:recursion} \\
     \Hstat{t}(x_t) &= \mathbb{E}^{\parvar,x_t}_{t-1|t}{\left[\Hstat{t-1}(X_{t-1}) + \addfelbo{t}(X_{t-1}, x_t)\right]}\\%\label{eq:Hstat:recursion}\\
     % \Gstat{t}(x_t) &= \mathbb{E}_{\vd{t-1|t}(x_{t},\cdot)}\left[\Gstat{t-1}\left(X_{t-1}\right) \right. \label{eq:Gstat:recursion}\\
     % &\left. 
     %  \hspace{1cm}+ \grad_\parvar \log \vd{t-1|t}(x_t, X_{t-1}) \right.\nonumber\\
     %  &\left. \hspace{1.5cm}\times\{\Hstat{t-1}(x_{t-1}) + \addfelbo{t}(x_{t-1}, x_t)
     % \} 
     % \right], \nonumber \\
     \Gstat{t}(x_t) &= \mathbb{E}^{\parvar,x_t}_{t-1|t}{\left[\Gstat{t-1}\left(X_{t-1}\right) + \grad_\parvar \log \vd{t-1|t}(x_t, X_{t-1}) \right.}\nonumber\\
      &{\left. \hspace{2.3cm}\times\{\Hstat{t-1}(x_{t-1}) + \addfelbo{t}(x_{t-1}, x_t)
     \} 
     \right]} \\%\label{eq:Gstat:recursion} \\
     % \Fstat{t}(x_t) &= \mathbb{E}_{\vd{t-1|t}(x_{t},\cdot)} \left[\Fstat{t-1}(X_{t-1}) + \grad_{\thp} \addfelbo{t}(X_{t-1}, x_t)\right]\eqsp, %\label{eq:Fstat:recursion}
     \Fstat{t}(x_t) &= \mathbb{E}^{\parvar,x_t}_{t-1|t} {\left[\Fstat{t-1}(X_{t-1}) + \grad_{\thp} \addfelbo{t}(X_{t-1}, x_t)\right]}\eqsp, %\label{eq:Fstat:recursion}
\end{align*}
with $\Hstat{0}(x_0) = \addfelbo{0}(x_{-1}, x_{0}),\Gstat{0}(x_0) = 0,$ and $\Fstat{0}(x_0)=\grad_\thp\addfelbo{0}(x_{-1}, x_{0})$. 
\end{proposition}

\begin{proof}
The proof is postponed to Appendix~\ref{appdx:proof:prp:elbo:recursion}. 
\end{proof}

In the light of Proposition~\ref{prp:elbo:grad:recursion}, given the observation record $y_{0:t}$, recursive computation of $\grad_\parvar \ELBO{t}$ consists, ideally, of (i) computing recursively $\Hstat{s},\Gstat{s}, \Fstat{s}$ for $0 \leqslant s \leqslant  t$ and (ii) computing the final expectations. 
As these final expectations are w.r.t. the chosen variational distribution $\vd{t}$, standard Monte Carlo sampling can be used to approximate the same.
However, it remains to approximate online these three intermediate functions, which are conditional expectations w.r.t. the kernels $\vd{t-1\vert t}$. 
% Note that these kernels aim to approximate the true backward kernels $b_{t-1|t}$, which depend only on past observations $Y_{0:t-1}$ and are therefore susceptible to online learning.
